Beyond Templates: Revisiting Zero-Shot Remote Sensing through Meta-Prompting

Vision-language models (VLMs) have sparked growing interest in zero-shot Earth Observation (EO) downstream tasks, with further gains enabled by remote-sensing-adapted models. We examine this setting across 17 VLM variants and 12 remote sensing (RS) datasets under Meta-Prompting for Visual Recognition (MPVR), and show that zero-shot performance remains highly sensitive to textual design choices, from the meta-prompts used to guide the LLM in generating class descriptions to the descriptions themselves. We explore why semantically rich LLM-generated class descriptions do not translate into consistent gains over simple domain-adapted CLIP-style descriptions. While LLM descriptions are more semantically expressive, they can also introduce noise in the text embedding space, reducing robustness in downstream tasks. We support this observation through a text log-likelihood analysis in the whitened CLIP feature space, comparing LLM-generated and template-based descriptions. Building on this finding, we study query embedding calibration and show that lightweight calibration of the query space consistently yields strong improvements in zero-shot classification and retrieval. Overall, our results provide practical insight into the trade-off between semantic richness and robustness, and identify embedding calibration as a simple and effective tool for improving zero-shot remote sensing performance.

==> plots/violin_clas/aid.tex <==
% ======================================================
% Baseline (x-axis at y=0)
% ======================================================
\addplot[
    name path=baseline,
    draw=none
]
coordinates {(67.06,0) (91.48,0)};

% ======================================================
% DEFAULT
% ======================================================

% ---- DS-Temp (top half) ----
\addplot[
    name path=ds_default_top,
    smooth,
    draw=\dstempcol,
    dashed,
    line width=0.8pt
] coordinates {
    ({67.06 - \dx}, 0.000000)
    ({69.50 - \dx}, 0.240883)
    ({74.39 - \dx}, 0.481765)
    ({79.27 - \dx}, 0.120441)
    ({84.15 - \dx}, 0.060221)
    ({89.04 - \dx}, 0.120441)
    ({91.48 - \dx}, 0.000000)
};

\addplot[
    fill=\dstempcol,
    fill opacity=0.2,
]
fill between[
    of=ds_default_top and baseline
];
\addplot[
    draw=\dstempcol,
    dashed,
    dash pattern=on 2pt off 1.4pt,
    dash phase=0pt,
    line width=0.5pt
] coordinates {
    ({75.47 - \dx},0) ({75.47 - \dx},0.900000)
};

% ---- LLaMA (bottom half) ----
\addplot[
    name path=llama_default_bot,
    smooth,
    draw=\llamacol,
    dashed,
    line width=0.8pt
] coordinates {
    ({67.06 - \dx}, -0.000000)
    ({69.50 - \dx}, -0.481765)
    ({74.39 - \dx}, -0.361324)
    ({79.27 - \dx}, -0.060221)
    ({84.15 - \dx}, -0.060221)
    ({89.04 - \dx}, -0.060221)
    ({91.48 - \dx}, -0.000000)
};

\addplot[
    fill=\llamacol,
    fill opacity=0.2,
]
fill between[
    of=llama_default_bot and baseline
];
\addplot[
    draw=\llamacol,
    dashed,
    dash pattern=on 2pt off 1.4pt,
    dash phase=0pt,
    line width=0.5pt
] coordinates {
    ({73.90 - \dx},0) ({73.90 - \dx},-0.900000)
};

% ======================================================
% CENTERED
% ======================================================

% ---- DS-Temp (top half) ----
\addplot[
    name path=ds_white_top,
    smooth,
    draw=\dstempcol,
    solid,
    line width=1.2pt
] coordinates {
    ({67.06 + \dx}, 0.000000)
    ({69.50 + \dx}, 0.481765)
    ({74.39 + \dx}, 0.361324)
    ({79.27 + \dx}, 0.000000)
    ({84.15 + \dx}, 0.060221)
    ({89.04 + \dx}, 0.120441)
    ({91.48 + \dx}, 0.000000)
};

\addplot[
    fill=\dstempcol,
    fill opacity=0.4,
]
fill between[
    of=ds_white_top and baseline
];
\addplot[
    draw=\dstempcol,
    solid,
    line width=0.5pt
] coordinates {
    ({74.21 + \dx},0) ({74.21 + \dx},0.900000)
};

% ---- LLaMA (bottom half) ----
\addplot[
    name path=llama_white_bot,
    smooth,
    draw=\llamacol,
    solid,
    line width=1.2pt
] coordinates {
    ({67.06 + \dx}, -0.000000)
    ({69.50 + \dx}, -0.602206)
    ({74.39 + \dx}, -0.301103)
    ({79.27 + \dx}, -0.060221)
    ({84.15 + \dx}, -0.060221)
    ({89.04 + \dx}, -0.000000)
    ({91.48 + \dx}, -0.000000)
};

\addplot[
    fill=\llamacol,
    fill opacity=0.4,
]
fill between[
    of=llama_white_bot and baseline
];
\addplot[
    draw=\llamacol,
    solid,
    line width=0.5pt
] coordinates {
    ({71.81 + \dx},0) ({71.81 + \dx},-0.900000)
};


==> plots/violin_clas/eurosat.tex <==
% ======================================================
% Baseline (x-axis at y=0)
% ======================================================
\addplot[
    name path=baseline,
    draw=none
]
coordinates {(23.17,0) (73.41,0)};

% ======================================================
% DEFAULT
% ======================================================

% ---- DS-Temp (top half) ----
\addplot[
    name path=ds_default_top,
    smooth,
    draw=\dstempcol,
    dashed,
    line width=0.8pt
] coordinates {
    ({23.17 - \dx}, 0.000000)
    ({28.19 - \dx}, 0.029271)
    ({38.24 - \dx}, 0.058543)
    ({48.29 - \dx}, 0.204899)
    ({58.34 - \dx}, 0.117085)
    ({68.39 - \dx}, 0.087814)
    ({73.41 - \dx}, 0.000000)
};

\addplot[
    fill=\dstempcol,
    fill opacity=0.2,
]
fill between[
    of=ds_default_top and baseline
];
\addplot[
    draw=\dstempcol,
    dashed,
    dash pattern=on 2pt off 1.4pt,
    dash phase=0pt,
    line width=0.5pt
] coordinates {
    ({51.70 - \dx},0) ({51.70 - \dx},0.900000)
};

% ---- LLaMA (bottom half) ----
\addplot[
    name path=llama_default_bot,
    smooth,
    draw=\llamacol,
    dashed,
    line width=0.8pt
] coordinates {
    ({23.17 - \dx}, -0.000000)
    ({28.19 - \dx}, -0.029271)
    ({38.24 - \dx}, -0.087814)
    ({48.29 - \dx}, -0.146356)
    ({58.34 - \dx}, -0.146356)
    ({68.39 - \dx}, -0.087814)
    ({73.41 - \dx}, -0.000000)
};

\addplot[
    fill=\llamacol,
    fill opacity=0.2,
]
fill between[
    of=llama_default_bot and baseline
];
\addplot[
    draw=\llamacol,
    dashed,
    dash pattern=on 2pt off 1.4pt,
    dash phase=0pt,
    line width=0.5pt
] coordinates {
    ({51.77 - \dx},0) ({51.77 - \dx},-0.900000)
};

% ======================================================
% CENTERED
% ======================================================

% ---- DS-Temp (top half) ----
\addplot[
    name path=ds_white_top,
    smooth,
    draw=\dstempcol,
    solid,
    line width=1.2pt
] coordinates {
    ({23.17 + \dx}, 0.000000)
    ({28.19 + \dx}, 0.029271)
    ({38.24 + \dx}, 0.029271)
    ({48.29 + \dx}, 0.087814)
    ({58.34 + \dx}, 0.204899)
    ({68.39 + \dx}, 0.146356)
    ({73.41 + \dx}, 0.000000)
};

\addplot[
    fill=\dstempcol,
    fill opacity=0.4,
]
fill between[
    of=ds_white_top and baseline
];
\addplot[
    draw=\dstempcol,
    solid,
    line width=0.5pt
] coordinates {
    ({55.31 + \dx},0) ({55.31 + \dx},0.900000)
};

% ---- LLaMA (bottom half) ----
\addplot[
    name path=llama_white_bot,
    smooth,
    draw=\llamacol,
    solid,
    line width=1.2pt
] coordinates {
    ({23.17 + \dx}, -0.000000)
    ({28.19 + \dx}, -0.029271)
    ({38.24 + \dx}, -0.000000)
    ({48.29 + \dx}, -0.146356)
    ({58.34 + \dx}, -0.175628)
    ({68.39 + \dx}, -0.146356)
    ({73.41 + \dx}, -0.000000)
};

\addplot[
    fill=\llamacol,
    fill opacity=0.4,
]
fill between[
    of=llama_white_bot and baseline
];
\addplot[
    draw=\llamacol,
    solid,
    line width=0.5pt
] coordinates {
    ({56.94 + \dx},0) ({56.94 + \dx},-0.900000)
};


==> plots/violin_clas/mlrsnet.tex <==
% ======================================================
% Baseline (x-axis at y=0)
% ======================================================
\addplot[
    name path=baseline,
    draw=none
]
coordinates {(42.28,0) (70.72,0)};

% ======================================================
% DEFAULT
% ======================================================

% ---- DS-Temp (top half) ----
\addplot[
    name path=ds_default_top,
    smooth,
    draw=\dstempcol,
    dashed,
    line width=0.8pt
] coordinates {
    ({42.28 - \dx}, 0.000000)
    ({45.12 - \dx}, 0.051708)
    ({50.81 - \dx}, 0.000000)
    ({56.50 - \dx}, 0.155125)
    ({62.19 - \dx}, 0.361959)
    ({67.88 - \dx}, 0.310251)
    ({70.72 - \dx}, 0.000000)
};

\addplot[
    fill=\dstempcol,
    fill opacity=0.2,
]
fill between[
    of=ds_default_top and baseline
];
\addplot[
    draw=\dstempcol,
    dashed,
    dash pattern=on 2pt off 1.4pt,
    dash phase=0pt,
    line width=0.5pt
] coordinates {
    ({62.21 - \dx},0) ({62.21 - \dx},0.900000)
};

% ---- LLaMA (bottom half) ----
\addplot[
    name path=llama_default_bot,
    smooth,
    draw=\llamacol,
    dashed,
    line width=0.8pt
] coordinates {
    ({42.28 - \dx}, -0.000000)
    ({45.12 - \dx}, -0.051708)
    ({50.81 - \dx}, -0.000000)
    ({56.50 - \dx}, -0.206834)
    ({62.19 - \dx}, -0.361959)
    ({67.88 - \dx}, -0.258542)
    ({70.72 - \dx}, -0.000000)
};

\addplot[
    fill=\llamacol,
    fill opacity=0.2,
]
fill between[
    of=llama_default_bot and baseline
];
\addplot[
    draw=\llamacol,
    dashed,
    dash pattern=on 2pt off 1.4pt,
    dash phase=0pt,
    line width=0.5pt
] coordinates {
    ({62.12 - \dx},0) ({62.12 - \dx},-0.900000)
};

% ======================================================
% CENTERED
% ======================================================

% ---- DS-Temp (top half) ----
\addplot[
    name path=ds_white_top,
    smooth,
    draw=\dstempcol,
    solid,
    line width=1.2pt
] coordinates {
    ({42.28 + \dx}, 0.000000)
    ({45.12 + \dx}, 0.000000)
    ({50.81 + \dx}, 0.051708)
    ({56.50 + \dx}, 0.103417)
    ({62.19 + \dx}, 0.413668)
    ({67.88 + \dx}, 0.310251)
    ({70.72 + \dx}, 0.000000)
};

\addplot[
    fill=\dstempcol,
    fill opacity=0.4,
]
fill between[
    of=ds_white_top and baseline
];
\addplot[
    draw=\dstempcol,
    solid,
    line width=0.5pt
] coordinates {
    ({63.24 + \dx},0) ({63.24 + \dx},0.900000)
};

% ---- LLaMA (bottom half) ----
\addplot[
    name path=llama_white_bot,
    smooth,
    draw=\llamacol,
    solid,
    line width=1.2pt
] coordinates {
    ({42.28 + \dx}, -0.000000)
    ({45.12 + \dx}, -0.000000)
    ({50.81 + \dx}, -0.051708)
    ({56.50 + \dx}, -0.103417)
    ({62.19 + \dx}, -0.465376)
    ({67.88 + \dx}, -0.258542)
    ({70.72 + \dx}, -0.000000)
};

\addplot[
    fill=\llamacol,
    fill opacity=0.4,
]
fill between[
    of=llama_white_bot and baseline
];
\addplot[
    draw=\llamacol,
    solid,
    line width=0.5pt
] coordinates {
    ({62.94 + \dx},0) ({62.94 + \dx},-0.900000)
};


==> plots/violin_clas/optimal31.tex <==
% ======================================================
% Baseline (x-axis at y=0)
% ======================================================
\addplot[
    name path=baseline,
    draw=none
]
coordinates {(63.76,0) (86.45,0)};

% ======================================================
% DEFAULT
% ======================================================

% ---- DS-Temp (top half) ----
\addplot[
    name path=ds_default_top,
    smooth,
    draw=\dstempcol,
    dashed,
    line width=0.8pt
] coordinates {
    ({63.76 - \dx}, 0.000000)
    ({66.03 - \dx}, 0.064812)
    ({70.57 - \dx}, 0.064812)
    ({75.10 - \dx}, 0.129624)
    ({79.64 - \dx}, 0.324061)
    ({84.18 - \dx}, 0.518497)
    ({86.45 - \dx}, 0.000000)
};

\addplot[
    fill=\dstempcol,
    fill opacity=0.2,
]
fill between[
    of=ds_default_top and baseline
];
\addplot[
    draw=\dstempcol,
    dashed,
    dash pattern=on 2pt off 1.4pt,
    dash phase=0pt,
    line width=0.5pt
] coordinates {
    ({79.65 - \dx},0) ({79.65 - \dx},0.900000)
};

% ---- LLaMA (bottom half) ----
\addplot[
    name path=llama_default_bot,
    smooth,
    draw=\llamacol,
    dashed,
    line width=0.8pt
] coordinates {
    ({63.76 - \dx}, -0.000000)
    ({66.03 - \dx}, -0.000000)
    ({70.57 - \dx}, -0.064812)
    ({75.10 - \dx}, -0.129624)
    ({79.64 - \dx}, -0.648122)
    ({84.18 - \dx}, -0.259249)
    ({86.45 - \dx}, -0.000000)
};

\addplot[
    fill=\llamacol,
    fill opacity=0.2,
]
fill between[
    of=llama_default_bot and baseline
];
\addplot[
    draw=\llamacol,
    dashed,
    dash pattern=on 2pt off 1.4pt,
    dash phase=0pt,
    line width=0.5pt
] coordinates {
    ({79.72 - \dx},0) ({79.72 - \dx},-0.900000)
};

% ======================================================
% CENTERED
% ======================================================

% ---- DS-Temp (top half) ----
\addplot[
    name path=ds_white_top,
    smooth,
    draw=\dstempcol,
    solid,
    line width=1.2pt
] coordinates {
    ({63.76 + \dx}, 0.000000)
    ({66.03 + \dx}, 0.064812)
    ({70.57 + \dx}, 0.000000)
    ({75.10 + \dx}, 0.194437)
    ({79.64 + \dx}, 0.648122)
    ({84.18 + \dx}, 0.194437)
    ({86.45 + \dx}, 0.000000)
};

\addplot[
    fill=\dstempcol,
    fill opacity=0.4,
]
fill between[
    of=ds_white_top and baseline
];
\addplot[
    draw=\dstempcol,
    solid,
    line width=0.5pt
] coordinates {
    ({78.94 + \dx},0) ({78.94 + \dx},0.900000)
};

% ---- LLaMA (bottom half) ----
\addplot[
    name path=llama_white_bot,
    smooth,
    draw=\llamacol,
    solid,
    line width=1.2pt
] coordinates {
    ({63.76 + \dx}, -0.000000)
    ({66.03 + \dx}, -0.000000)
    ({70.57 + \dx}, -0.064812)
    ({75.10 + \dx}, -0.259249)
    ({79.64 + \dx}, -0.453685)
    ({84.18 + \dx}, -0.324061)
    ({86.45 + \dx}, -0.000000)
};

\addplot[
    fill=\llamacol,
    fill opacity=0.4,
]
fill between[
    of=llama_white_bot and baseline
];
\addplot[
    draw=\llamacol,
    solid,
    line width=0.5pt
] coordinates {
    ({79.50 + \dx},0) ({79.50 + \dx},-0.900000)
};


==> plots/violin_clas/patternnet.tex <==
% ======================================================
% Baseline (x-axis at y=0)
% ======================================================
\addplot[
    name path=baseline,
    draw=none
]
coordinates {(45.86,0) (85.62,0)};

% ======================================================
% DEFAULT
% ======================================================

% ---- DS-Temp (top half) ----
\addplot[
    name path=ds_default_top,
    smooth,
    draw=\dstempcol,
    dashed,
    line width=0.8pt
] coordinates {
    ({45.86 - \dx}, 0.000000)
    ({49.84 - \dx}, 0.036987)
    ({57.79 - \dx}, 0.036987)
    ({65.74 - \dx}, 0.184933)
    ({73.69 - \dx}, 0.184933)
    ({81.64 - \dx}, 0.184933)
    ({85.62 - \dx}, 0.000000)
};

\addplot[
    fill=\dstempcol,
    fill opacity=0.2,
]
fill between[
    of=ds_default_top and baseline
];
\addplot[
    draw=\dstempcol,
    dashed,
    dash pattern=on 2pt off 1.4pt,
    dash phase=0pt,
    line width=0.5pt
] coordinates {
    ({70.78 - \dx},0) ({70.78 - \dx},0.900000)
};

% ---- LLaMA (bottom half) ----
\addplot[
    name path=llama_default_bot,
    smooth,
    draw=\llamacol,
    dashed,
    line width=0.8pt
] coordinates {
    ({45.86 - \dx}, -0.000000)
    ({49.84 - \dx}, -0.036987)
    ({57.79 - \dx}, -0.036987)
    ({65.74 - \dx}, -0.110960)
    ({73.69 - \dx}, -0.295893)
    ({81.64 - \dx}, -0.147947)
    ({85.62 - \dx}, -0.000000)
};

\addplot[
    fill=\llamacol,
    fill opacity=0.2,
]
fill between[
    of=llama_default_bot and baseline
];
\addplot[
    draw=\llamacol,
    dashed,
    dash pattern=on 2pt off 1.4pt,
    dash phase=0pt,
    line width=0.5pt
] coordinates {
    ({71.53 - \dx},0) ({71.53 - \dx},-0.900000)
};

% ======================================================
% CENTERED
% ======================================================

% ---- DS-Temp (top half) ----
\addplot[
    name path=ds_white_top,
    smooth,
    draw=\dstempcol,
    solid,
    line width=1.2pt
] coordinates {
    ({45.86 + \dx}, 0.000000)
    ({49.84 + \dx}, 0.036987)
    ({57.79 + \dx}, 0.036987)
    ({65.74 + \dx}, 0.110960)
    ({73.69 + \dx}, 0.221920)
    ({81.64 + \dx}, 0.221920)
    ({85.62 + \dx}, 0.000000)
};

\addplot[
    fill=\dstempcol,
    fill opacity=0.4,
]
fill between[
    of=ds_white_top and baseline
];
\addplot[
    draw=\dstempcol,
    solid,
    line width=0.5pt
] coordinates {
    ({72.40 + \dx},0) ({72.40 + \dx},0.900000)
};

% ---- LLaMA (bottom half) ----
\addplot[
    name path=llama_white_bot,
    smooth,
    draw=\llamacol,
    solid,
    line width=1.2pt
] coordinates {
    ({45.86 + \dx}, -0.000000)
    ({49.84 + \dx}, -0.036987)
    ({57.79 + \dx}, -0.000000)
    ({65.74 + \dx}, -0.073973)
    ({73.69 + \dx}, -0.295893)
    ({81.64 + \dx}, -0.221920)
    ({85.62 + \dx}, -0.000000)
};

\addplot[
    fill=\llamacol,
    fill opacity=0.4,
]
fill between[
    of=llama_white_bot and baseline
];
\addplot[
    draw=\llamacol,
    solid,
    line width=0.5pt
] coordinates {
    ({73.54 + \dx},0) ({73.54 + \dx},-0.900000)
};


==> plots/violin_clas/resisc45.tex <==
% ======================================================
% Baseline (x-axis at y=0)
% ======================================================
\addplot[
    name path=baseline,
    draw=none
]
coordinates {(51.36,0) (75.40,0)};

% ======================================================
% DEFAULT
% ======================================================

% ---- DS-Temp (top half) ----
\addplot[
    name path=ds_default_top,
    smooth,
    draw=\dstempcol,
    dashed,
    line width=0.8pt
] coordinates {
    ({51.36 - \dx}, 0.000000)
    ({53.76 - \dx}, 0.061173)
    ({58.57 - \dx}, 0.000000)
    ({63.38 - \dx}, 0.122345)
    ({68.19 - \dx}, 0.305863)
    ({73.00 - \dx}, 0.550553)
    ({75.40 - \dx}, 0.000000)
};

\addplot[
    fill=\dstempcol,
    fill opacity=0.2,
]
fill between[
    of=ds_default_top and baseline
];
\addplot[
    draw=\dstempcol,
    dashed,
    dash pattern=on 2pt off 1.4pt,
    dash phase=0pt,
    line width=0.5pt
] coordinates {
    ({69.97 - \dx},0) ({69.97 - \dx},0.900000)
};

% ---- LLaMA (bottom half) ----
\addplot[
    name path=llama_default_bot,
    smooth,
    draw=\llamacol,
    dashed,
    line width=0.8pt
] coordinates {
    ({51.36 - \dx}, -0.000000)
    ({53.76 - \dx}, -0.000000)
    ({58.57 - \dx}, -0.061173)
    ({63.38 - \dx}, -0.000000)
    ({68.19 - \dx}, -0.367035)
    ({73.00 - \dx}, -0.611726)
    ({75.40 - \dx}, -0.000000)
};

\addplot[
    fill=\llamacol,
    fill opacity=0.2,
]
fill between[
    of=llama_default_bot and baseline
];
\addplot[
    draw=\llamacol,
    dashed,
    dash pattern=on 2pt off 1.4pt,
    dash phase=0pt,
    line width=0.5pt
] coordinates {
    ({70.32 - \dx},0) ({70.32 - \dx},-0.900000)
};

% ======================================================
% CENTERED
% ======================================================

% ---- DS-Temp (top half) ----
\addplot[
    name path=ds_white_top,
    smooth,
    draw=\dstempcol,
    solid,
    line width=1.2pt
] coordinates {
    ({51.36 + \dx}, 0.000000)
    ({53.76 + \dx}, 0.061173)
    ({58.57 + \dx}, 0.000000)
    ({63.38 + \dx}, 0.183518)
    ({68.19 + \dx}, 0.550553)
    ({73.00 + \dx}, 0.244690)
    ({75.40 + \dx}, 0.000000)
};

\addplot[
    fill=\dstempcol,
    fill opacity=0.4,
]
fill between[
    of=ds_white_top and baseline
];
\addplot[
    draw=\dstempcol,
    solid,
    line width=0.5pt
] coordinates {
    ({68.13 + \dx},0) ({68.13 + \dx},0.900000)
};

% ---- LLaMA (bottom half) ----
\addplot[
    name path=llama_white_bot,
    smooth,
    draw=\llamacol,
    solid,
    line width=1.2pt
] coordinates {
    ({51.36 + \dx}, -0.000000)
    ({53.76 + \dx}, -0.000000)
    ({58.57 + \dx}, -0.061173)
    ({63.38 + \dx}, -0.061173)
    ({68.19 + \dx}, -0.489380)
    ({73.00 + \dx}, -0.428208)
    ({75.40 + \dx}, -0.000000)
};

\addplot[
    fill=\llamacol,
    fill opacity=0.4,
]
fill between[
    of=llama_white_bot and baseline
];
\addplot[
    draw=\llamacol,
    solid,
    line width=0.5pt
] coordinates {
    ({69.81 + \dx},0) ({69.81 + \dx},-0.900000)
};


==> plots/violin_clas/rsc11.tex <==
% ======================================================
% Baseline (x-axis at y=0)
% ======================================================
\addplot[
    name path=baseline,
    draw=none
]
coordinates {(61.12,0) (82.01,0)};

% ======================================================
% DEFAULT
% ======================================================

% ---- DS-Temp (top half) ----
\addplot[
    name path=ds_default_top,
    smooth,
    draw=\dstempcol,
    dashed,
    line width=0.8pt
] coordinates {
    ({61.12 - \dx}, 0.000000)
    ({63.21 - \dx}, 0.703968)
    ({67.39 - \dx}, 0.281587)
    ({71.56 - \dx}, 0.070397)
    ({75.74 - \dx}, 0.070397)
    ({79.92 - \dx}, 0.070397)
    ({82.01 - \dx}, 0.000000)
};

\addplot[
    fill=\dstempcol,
    fill opacity=0.2,
]
fill between[
    of=ds_default_top and baseline
];
\addplot[
    draw=\dstempcol,
    dashed,
    dash pattern=on 2pt off 1.4pt,
    dash phase=0pt,
    line width=0.5pt
] coordinates {
    ({66.09 - \dx},0) ({66.09 - \dx},0.900000)
};

% ---- LLaMA (bottom half) ----
\addplot[
    name path=llama_default_bot,
    smooth,
    draw=\llamacol,
    dashed,
    line width=0.8pt
] coordinates {
    ({61.12 - \dx}, -0.000000)
    ({63.21 - \dx}, -0.422381)
    ({67.39 - \dx}, -0.351984)
    ({71.56 - \dx}, -0.351984)
    ({75.74 - \dx}, -0.070397)
    ({79.92 - \dx}, -0.000000)
    ({82.01 - \dx}, -0.000000)
};

\addplot[
    fill=\llamacol,
    fill opacity=0.2,
]
fill between[
    of=llama_default_bot and baseline
];
\addplot[
    draw=\llamacol,
    dashed,
    dash pattern=on 2pt off 1.4pt,
    dash phase=0pt,
    line width=0.5pt
] coordinates {
    ({67.68 - \dx},0) ({67.68 - \dx},-0.900000)
};

% ======================================================
% CENTERED
% ======================================================

% ---- DS-Temp (top half) ----
\addplot[
    name path=ds_white_top,
    smooth,
    draw=\dstempcol,
    solid,
    line width=1.2pt
] coordinates {
    ({61.12 + \dx}, 0.000000)
    ({63.21 + \dx}, 0.281587)
    ({67.39 + \dx}, 0.070397)
    ({71.56 + \dx}, 0.703968)
    ({75.74 + \dx}, 0.140794)
    ({79.92 + \dx}, 0.000000)
    ({82.01 + \dx}, 0.000000)
};

\addplot[
    fill=\dstempcol,
    fill opacity=0.4,
]
fill between[
    of=ds_white_top and baseline
];
\addplot[
    draw=\dstempcol,
    solid,
    line width=0.5pt
] coordinates {
    ({70.22 + \dx},0) ({70.22 + \dx},0.900000)
};

% ---- LLaMA (bottom half) ----
\addplot[
    name path=llama_white_bot,
    smooth,
    draw=\llamacol,
    solid,
    line width=1.2pt
] coordinates {
    ({61.12 + \dx}, -0.000000)
    ({63.21 + \dx}, -0.070397)
    ({67.39 + \dx}, -0.140794)
    ({71.56 + \dx}, -0.281587)
    ({75.74 + \dx}, -0.633571)
    ({79.92 + \dx}, -0.070397)
    ({82.01 + \dx}, -0.000000)
};

\addplot[
    fill=\llamacol,
    fill opacity=0.4,
]
fill between[
    of=llama_white_bot and baseline
];
\addplot[
    draw=\llamacol,
    solid,
    line width=0.5pt
] coordinates {
    ({73.50 + \dx},0) ({73.50 + \dx},-0.900000)
};


==> plots/violin_clas/rsicb128.tex <==
% ======================================================
% Baseline (x-axis at y=0)
% ======================================================
\addplot[
    name path=baseline,
    draw=none
]
coordinates {(16.32,0) (48.51,0)};

% ======================================================
% DEFAULT
% ======================================================

% ---- DS-Temp (top half) ----
\addplot[
    name path=ds_default_top,
    smooth,
    draw=\dstempcol,
    dashed,
    line width=0.8pt
] coordinates {
    ({16.32 - \dx}, 0.000000)
    ({19.54 - \dx}, 0.045685)
    ({25.98 - \dx}, 0.091369)
    ({32.41 - \dx}, 0.365477)
    ({38.85 - \dx}, 0.182739)
    ({45.29 - \dx}, 0.091369)
    ({48.51 - \dx}, 0.000000)
};

\addplot[
    fill=\dstempcol,
    fill opacity=0.2,
]
fill between[
    of=ds_default_top and baseline
];
\addplot[
    draw=\dstempcol,
    dashed,
    dash pattern=on 2pt off 1.4pt,
    dash phase=0pt,
    line width=0.5pt
] coordinates {
    ({34.24 - \dx},0) ({34.24 - \dx},0.900000)
};

% ---- LLaMA (bottom half) ----
\addplot[
    name path=llama_default_bot,
    smooth,
    draw=\llamacol,
    dashed,
    line width=0.8pt
] coordinates {
    ({16.32 - \dx}, -0.000000)
    ({19.54 - \dx}, -0.045685)
    ({25.98 - \dx}, -0.091369)
    ({32.41 - \dx}, -0.411162)
    ({38.85 - \dx}, -0.182739)
    ({45.29 - \dx}, -0.045685)
    ({48.51 - \dx}, -0.000000)
};

\addplot[
    fill=\llamacol,
    fill opacity=0.2,
]
fill between[
    of=llama_default_bot and baseline
];
\addplot[
    draw=\llamacol,
    dashed,
    dash pattern=on 2pt off 1.4pt,
    dash phase=0pt,
    line width=0.5pt
] coordinates {
    ({33.98 - \dx},0) ({33.98 - \dx},-0.900000)
};

% ======================================================
% CENTERED
% ======================================================

% ---- DS-Temp (top half) ----
\addplot[
    name path=ds_white_top,
    smooth,
    draw=\dstempcol,
    solid,
    line width=1.2pt
] coordinates {
    ({16.32 + \dx}, 0.000000)
    ({19.54 + \dx}, 0.045685)
    ({25.98 + \dx}, 0.091369)
    ({32.41 + \dx}, 0.182739)
    ({38.85 + \dx}, 0.365477)
    ({45.29 + \dx}, 0.091369)
    ({48.51 + \dx}, 0.000000)
};

\addplot[
    fill=\dstempcol,
    fill opacity=0.4,
]
fill between[
    of=ds_white_top and baseline
];
\addplot[
    draw=\dstempcol,
    solid,
    line width=0.5pt
] coordinates {
    ({35.45 + \dx},0) ({35.45 + \dx},0.900000)
};

% ---- LLaMA (bottom half) ----
\addplot[
    name path=llama_white_bot,
    smooth,
    draw=\llamacol,
    solid,
    line width=1.2pt
] coordinates {
    ({16.32 + \dx}, -0.000000)
    ({19.54 + \dx}, -0.000000)
    ({25.98 + \dx}, -0.045685)
    ({32.41 + \dx}, -0.182739)
    ({38.85 + \dx}, -0.365477)
    ({45.29 + \dx}, -0.182739)
    ({48.51 + \dx}, -0.000000)
};

\addplot[
    fill=\llamacol,
    fill opacity=0.4,
]
fill between[
    of=llama_white_bot and baseline
];
\addplot[
    draw=\llamacol,
    solid,
    line width=0.5pt
] coordinates {
    ({37.91 + \dx},0) ({37.91 + \dx},-0.900000)
};


==> plots/violin_clas/rsicb256.tex <==
% ======================================================
% Baseline (x-axis at y=0)
% ======================================================
\addplot[
    name path=baseline,
    draw=none
]
coordinates {(31.78,0) (59.65,0)};

% ======================================================
% DEFAULT
% ======================================================

% ---- DS-Temp (top half) ----
\addplot[
    name path=ds_default_top,
    smooth,
    draw=\dstempcol,
    dashed,
    line width=0.8pt
] coordinates {
    ({31.78 - \dx}, 0.000000)
    ({34.57 - \dx}, 0.105532)
    ({40.14 - \dx}, 0.263830)
    ({45.72 - \dx}, 0.263830)
    ({51.29 - \dx}, 0.211064)
    ({56.86 - \dx}, 0.052766)
    ({59.65 - \dx}, 0.000000)
};

\addplot[
    fill=\dstempcol,
    fill opacity=0.2,
]
fill between[
    of=ds_default_top and baseline
];
\addplot[
    draw=\dstempcol,
    dashed,
    dash pattern=on 2pt off 1.4pt,
    dash phase=0pt,
    line width=0.5pt
] coordinates {
    ({44.48 - \dx},0) ({44.48 - \dx},0.900000)
};

% ---- LLaMA (bottom half) ----
\addplot[
    name path=llama_default_bot,
    smooth,
    draw=\llamacol,
    dashed,
    line width=0.8pt
] coordinates {
    ({31.78 - \dx}, -0.000000)
    ({34.57 - \dx}, -0.105532)
    ({40.14 - \dx}, -0.369362)
    ({45.72 - \dx}, -0.105532)
    ({51.29 - \dx}, -0.316596)
    ({56.86 - \dx}, -0.000000)
    ({59.65 - \dx}, -0.000000)
};

\addplot[
    fill=\llamacol,
    fill opacity=0.2,
]
fill between[
    of=llama_default_bot and baseline
];
\addplot[
    draw=\llamacol,
    dashed,
    dash pattern=on 2pt off 1.4pt,
    dash phase=0pt,
    line width=0.5pt
] coordinates {
    ({43.92 - \dx},0) ({43.92 - \dx},-0.900000)
};

% ======================================================
% CENTERED
% ======================================================

% ---- DS-Temp (top half) ----
\addplot[
    name path=ds_white_top,
    smooth,
    draw=\dstempcol,
    solid,
    line width=1.2pt
] coordinates {
    ({31.78 + \dx}, 0.000000)
    ({34.57 + \dx}, 0.052766)
    ({40.14 + \dx}, 0.105532)
    ({45.72 + \dx}, 0.422128)
    ({51.29 + \dx}, 0.263830)
    ({56.86 + \dx}, 0.052766)
    ({59.65 + \dx}, 0.000000)
};

\addplot[
    fill=\dstempcol,
    fill opacity=0.4,
]
fill between[
    of=ds_white_top and baseline
];
\addplot[
    draw=\dstempcol,
    solid,
    line width=0.5pt
] coordinates {
    ({46.16 + \dx},0) ({46.16 + \dx},0.900000)
};

% ---- LLaMA (bottom half) ----
\addplot[
    name path=llama_white_bot,
    smooth,
    draw=\llamacol,
    solid,
    line width=1.2pt
] coordinates {
    ({31.78 + \dx}, -0.000000)
    ({34.57 + \dx}, -0.000000)
    ({40.14 + \dx}, -0.052766)
    ({45.72 + \dx}, -0.263830)
    ({51.29 + \dx}, -0.369362)
    ({56.86 + \dx}, -0.211064)
    ({59.65 + \dx}, -0.000000)
};

\addplot[
    fill=\llamacol,
    fill opacity=0.4,
]
fill between[
    of=llama_white_bot and baseline
];
\addplot[
    draw=\llamacol,
    solid,
    line width=0.5pt
] coordinates {
    ({50.02 + \dx},0) ({50.02 + \dx},-0.900000)
};


==> plots/violin_clas/rsscn7.tex <==
% ======================================================
% Baseline (x-axis at y=0)
% ======================================================
\addplot[
    name path=baseline,
    draw=none
]
coordinates {(49.46,0) (83.49,0)};

% ======================================================
% DEFAULT
% ======================================================

% ---- DS-Temp (top half) ----
\addplot[
    name path=ds_default_top,
    smooth,
    draw=\dstempcol,
    dashed,
    line width=0.8pt
] coordinates {
    ({49.46 - \dx}, 0.000000)
    ({52.86 - \dx}, 0.043214)
    ({59.67 - \dx}, 0.043214)
    ({66.47 - \dx}, 0.518574)
    ({73.28 - \dx}, 0.086429)
    ({80.09 - \dx}, 0.043214)
    ({83.49 - \dx}, 0.000000)
};

\addplot[
    fill=\dstempcol,
    fill opacity=0.2,
]
fill between[
    of=ds_default_top and baseline
];
\addplot[
    draw=\dstempcol,
    dashed,
    dash pattern=on 2pt off 1.4pt,
    dash phase=0pt,
    line width=0.5pt
] coordinates {
    ({66.64 - \dx},0) ({66.64 - \dx},0.900000)
};

% ---- LLaMA (bottom half) ----
\addplot[
    name path=llama_default_bot,
    smooth,
    draw=\llamacol,
    dashed,
    line width=0.8pt
] coordinates {
    ({49.46 - \dx}, -0.000000)
    ({52.86 - \dx}, -0.000000)
    ({59.67 - \dx}, -0.000000)
    ({66.47 - \dx}, -0.216072)
    ({73.28 - \dx}, -0.432145)
    ({80.09 - \dx}, -0.086429)
    ({83.49 - \dx}, -0.000000)
};

\addplot[
    fill=\llamacol,
    fill opacity=0.2,
]
fill between[
    of=llama_default_bot and baseline
];
\addplot[
    draw=\llamacol,
    dashed,
    dash pattern=on 2pt off 1.4pt,
    dash phase=0pt,
    line width=0.5pt
] coordinates {
    ({71.70 - \dx},0) ({71.70 - \dx},-0.900000)
};

% ======================================================
% CENTERED
% ======================================================

% ---- DS-Temp (top half) ----
\addplot[
    name path=ds_white_top,
    smooth,
    draw=\dstempcol,
    solid,
    line width=1.2pt
] coordinates {
    ({49.46 + \dx}, 0.000000)
    ({52.86 + \dx}, 0.043214)
    ({59.67 + \dx}, 0.000000)
    ({66.47 + \dx}, 0.172858)
    ({73.28 + \dx}, 0.432145)
    ({80.09 + \dx}, 0.086429)
    ({83.49 + \dx}, 0.000000)
};

\addplot[
    fill=\dstempcol,
    fill opacity=0.4,
]
fill between[
    of=ds_white_top and baseline
];
\addplot[
    draw=\dstempcol,
    solid,
    line width=0.5pt
] coordinates {
    ({71.27 + \dx},0) ({71.27 + \dx},0.900000)
};

% ---- LLaMA (bottom half) ----
\addplot[
    name path=llama_white_bot,
    smooth,
    draw=\llamacol,
    solid,
    line width=1.2pt
] coordinates {
    ({49.46 + \dx}, -0.000000)
    ({52.86 + \dx}, -0.000000)
    ({59.67 + \dx}, -0.000000)
    ({66.47 + \dx}, -0.000000)
    ({73.28 + \dx}, -0.259287)
    ({80.09 + \dx}, -0.475359)
    ({83.49 + \dx}, -0.000000)
};

\addplot[
    fill=\llamacol,
    fill opacity=0.4,
]
fill between[
    of=llama_white_bot and baseline
];
\addplot[
    draw=\llamacol,
    solid,
    line width=0.5pt
] coordinates {
    ({77.29 + \dx},0) ({77.29 + \dx},-0.900000)
};


==> plots/violin_clas/siriwhu.tex <==
% ======================================================
% Baseline (x-axis at y=0)
% ======================================================
\addplot[
    name path=baseline,
    draw=none
]
coordinates {(52.90,0) (72.64,0)};

% ======================================================
% DEFAULT
% ======================================================

% ---- DS-Temp (top half) ----
\addplot[
    name path=ds_default_top,
    smooth,
    draw=\dstempcol,
    dashed,
    line width=0.8pt
] coordinates {
    ({52.90 - \dx}, 0.000000)
    ({54.87 - \dx}, 0.148996)
    ({58.82 - \dx}, 0.223494)
    ({62.77 - \dx}, 0.372489)
    ({66.72 - \dx}, 0.521485)
    ({70.67 - \dx}, 0.000000)
    ({72.64 - \dx}, 0.000000)
};

\addplot[
    fill=\dstempcol,
    fill opacity=0.2,
]
fill between[
    of=ds_default_top and baseline
];
\addplot[
    draw=\dstempcol,
    dashed,
    dash pattern=on 2pt off 1.4pt,
    dash phase=0pt,
    line width=0.5pt
] coordinates {
    ({63.00 - \dx},0) ({63.00 - \dx},0.900000)
};

% ---- LLaMA (bottom half) ----
\addplot[
    name path=llama_default_bot,
    smooth,
    draw=\llamacol,
    dashed,
    line width=0.8pt
] coordinates {
    ({52.90 - \dx}, -0.000000)
    ({54.87 - \dx}, -0.223494)
    ({58.82 - \dx}, -0.521485)
    ({62.77 - \dx}, -0.372489)
    ({66.72 - \dx}, -0.074498)
    ({70.67 - \dx}, -0.074498)
    ({72.64 - \dx}, -0.000000)
};

\addplot[
    fill=\llamacol,
    fill opacity=0.2,
]
fill between[
    of=llama_default_bot and baseline
];
\addplot[
    draw=\llamacol,
    dashed,
    dash pattern=on 2pt off 1.4pt,
    dash phase=0pt,
    line width=0.5pt
] coordinates {
    ({60.09 - \dx},0) ({60.09 - \dx},-0.900000)
};

% ======================================================
% CENTERED
% ======================================================

% ---- DS-Temp (top half) ----
\addplot[
    name path=ds_white_top,
    smooth,
    draw=\dstempcol,
    solid,
    line width=1.2pt
] coordinates {
    ({52.90 + \dx}, 0.000000)
    ({54.87 + \dx}, 0.000000)
    ({58.82 + \dx}, 0.074498)
    ({62.77 + \dx}, 0.297992)
    ({66.72 + \dx}, 0.670481)
    ({70.67 + \dx}, 0.223494)
    ({72.64 + \dx}, 0.000000)
};

\addplot[
    fill=\dstempcol,
    fill opacity=0.4,
]
fill between[
    of=ds_white_top and baseline
];
\addplot[
    draw=\dstempcol,
    solid,
    line width=0.5pt
] coordinates {
    ({66.07 + \dx},0) ({66.07 + \dx},0.900000)
};

% ---- LLaMA (bottom half) ----
\addplot[
    name path=llama_white_bot,
    smooth,
    draw=\llamacol,
    solid,
    line width=1.2pt
] coordinates {
    ({52.90 + \dx}, -0.000000)
    ({54.87 + \dx}, -0.000000)
    ({58.82 + \dx}, -0.074498)
    ({62.77 + \dx}, -0.223494)
    ({66.72 + \dx}, -0.595983)
    ({70.67 + \dx}, -0.372489)
    ({72.64 + \dx}, -0.000000)
};

\addplot[
    fill=\llamacol,
    fill opacity=0.4,
]
fill between[
    of=llama_white_bot and baseline
];
\addplot[
    draw=\llamacol,
    solid,
    line width=0.5pt
] coordinates {
    ({66.53 + \dx},0) ({66.53 + \dx},-0.900000)
};


==> plots/violin_clas/whurs19.tex <==
% ======================================================
% Baseline (x-axis at y=0)
% ======================================================
\addplot[
    name path=baseline,
    draw=none
]
coordinates {(82.29,0) (95.29,0)};

% ======================================================
% DEFAULT
% ======================================================

% ---- DS-Temp (top half) ----
\addplot[
    name path=ds_default_top,
    smooth,
    draw=\dstempcol,
    dashed,
    line width=0.8pt
] coordinates {
    ({82.29 - \dx}, 0.000000)
    ({83.59 - \dx}, 0.000000)
    ({86.19 - \dx}, 0.339367)
    ({88.79 - \dx}, 0.565611)
    ({91.39 - \dx}, 0.565611)
    ({93.99 - \dx}, 0.452489)
    ({95.29 - \dx}, 0.000000)
};

\addplot[
    fill=\dstempcol,
    fill opacity=0.2,
]
fill between[
    of=ds_default_top and baseline
];
\addplot[
    draw=\dstempcol,
    dashed,
    dash pattern=on 2pt off 1.4pt,
    dash phase=0pt,
    line width=0.5pt
] coordinates {
    ({90.11 - \dx},0) ({90.11 - \dx},0.900000)
};

% ---- LLaMA (bottom half) ----
\addplot[
    name path=llama_default_bot,
    smooth,
    draw=\llamacol,
    dashed,
    line width=0.8pt
] coordinates {
    ({82.29 - \dx}, -0.000000)
    ({83.59 - \dx}, -0.113122)
    ({86.19 - \dx}, -0.339367)
    ({88.79 - \dx}, -0.678733)
    ({91.39 - \dx}, -0.565611)
    ({93.99 - \dx}, -0.226244)
    ({95.29 - \dx}, -0.000000)
};

\addplot[
    fill=\llamacol,
    fill opacity=0.2,
]
fill between[
    of=llama_default_bot and baseline
];
\addplot[
    draw=\llamacol,
    dashed,
    dash pattern=on 2pt off 1.4pt,
    dash phase=0pt,
    line width=0.5pt
] coordinates {
    ({89.64 - \dx},0) ({89.64 - \dx},-0.900000)
};

% ======================================================
% CENTERED
% ======================================================

% ---- DS-Temp (top half) ----
\addplot[
    name path=ds_white_top,
    smooth,
    draw=\dstempcol,
    solid,
    line width=1.2pt
] coordinates {
    ({82.29 + \dx}, 0.000000)
    ({83.59 + \dx}, 0.113122)
    ({86.19 + \dx}, 0.452489)
    ({88.79 + \dx}, 0.791855)
    ({91.39 + \dx}, 0.226244)
    ({93.99 + \dx}, 0.339367)
    ({95.29 + \dx}, 0.000000)
};

\addplot[
    fill=\dstempcol,
    fill opacity=0.4,
]
fill between[
    of=ds_white_top and baseline
];
\addplot[
    draw=\dstempcol,
    solid,
    line width=0.5pt
] coordinates {
    ({89.27 + \dx},0) ({89.27 + \dx},0.900000)
};

% ---- LLaMA (bottom half) ----
\addplot[
    name path=llama_white_bot,
    smooth,
    draw=\llamacol,
    solid,
    line width=1.2pt
] coordinates {
    ({82.29 + \dx}, -0.000000)
    ({83.59 + \dx}, -0.113122)
    ({86.19 + \dx}, -0.452489)
    ({88.79 + \dx}, -0.791855)
    ({91.39 + \dx}, -0.452489)
    ({93.99 + \dx}, -0.113122)
    ({95.29 + \dx}, -0.000000)
};

\addplot[
    fill=\llamacol,
    fill opacity=0.4,
]
fill between[
    of=llama_white_bot and baseline
];
\addplot[
    draw=\llamacol,
    solid,
    line width=0.5pt
] coordinates {
    ({89.04 + \dx},0) ({89.04 + \dx},-0.900000)
};


==> plots/violin_ret/aid.tex <==
% ======================================================
% Baseline (x-axis at y=0)
% ======================================================
\addplot[
    name path=baseline,
    draw=none
]
coordinates {(49.94,0) (90.88,0)};

% ======================================================
% DEFAULT
% ======================================================

% ---- DS-Temp (top half) ----
\addplot[
    name path=ds_default_top,
    smooth,
    draw=\dstempcol,
    dashed,
    line width=0.8pt
] coordinates {
    ({49.94 - \dx}, 0.000000)
    ({54.03 - \dx}, 0.035921)
    ({62.22 - \dx}, 0.107762)
    ({70.41 - \dx}, 0.395126)
    ({78.60 - \dx}, 0.071841)
    ({86.79 - \dx}, 0.000000)
    ({90.88 - \dx}, 0.000000)
};

\addplot[
    fill=\dstempcol,
    fill opacity=0.2,
]
fill between[
    of=ds_default_top and baseline
];
\addplot[
    draw=\dstempcol,
    dashed,
    dash pattern=on 2pt off 1.4pt,
    dash phase=0pt,
    line width=0.5pt
] coordinates {
    ({69.17 - \dx},0) ({69.17 - \dx},0.900000)
};

% ---- LLaMA (bottom half) ----
\addplot[
    name path=llama_default_bot,
    smooth,
    draw=\llamacol,
    dashed,
    line width=0.8pt
] coordinates {
    ({49.94 - \dx}, -0.000000)
    ({54.03 - \dx}, -0.071841)
    ({62.22 - \dx}, -0.431047)
    ({70.41 - \dx}, -0.107762)
    ({78.60 - \dx}, -0.000000)
    ({86.79 - \dx}, -0.000000)
    ({90.88 - \dx}, -0.000000)
};

\addplot[
    fill=\llamacol,
    fill opacity=0.2,
]
fill between[
    of=llama_default_bot and baseline
];
\addplot[
    draw=\llamacol,
    dashed,
    dash pattern=on 2pt off 1.4pt,
    dash phase=0pt,
    line width=0.5pt
] coordinates {
    ({63.05 - \dx},0) ({63.05 - \dx},-0.900000)
};

% ======================================================
% CENTERED
% ======================================================

% ---- DS-Temp (top half) ----
\addplot[
    name path=ds_white_top,
    smooth,
    draw=\dstempcol,
    solid,
    line width=1.2pt
] coordinates {
    ({49.94 + \dx}, 0.000000)
    ({54.03 + \dx}, 0.000000)
    ({62.22 + \dx}, 0.000000)
    ({70.41 + \dx}, 0.431047)
    ({78.60 + \dx}, 0.071841)
    ({86.79 + \dx}, 0.107762)
    ({90.88 + \dx}, 0.000000)
};

\addplot[
    fill=\dstempcol,
    fill opacity=0.4,
]
fill between[
    of=ds_white_top and baseline
];
\addplot[
    draw=\dstempcol,
    solid,
    line width=0.5pt
] coordinates {
    ({75.24 + \dx},0) ({75.24 + \dx},0.900000)
};

% ---- LLaMA (bottom half) ----
\addplot[
    name path=llama_white_bot,
    smooth,
    draw=\llamacol,
    solid,
    line width=1.2pt
] coordinates {
    ({49.94 + \dx}, -0.000000)
    ({54.03 + \dx}, -0.000000)
    ({62.22 + \dx}, -0.000000)
    ({70.41 + \dx}, -0.502888)
    ({78.60 + \dx}, -0.071841)
    ({86.79 + \dx}, -0.035921)
    ({90.88 + \dx}, -0.000000)
};

\addplot[
    fill=\llamacol,
    fill opacity=0.4,
]
fill between[
    of=llama_white_bot and baseline
];
\addplot[
    draw=\llamacol,
    solid,
    line width=0.5pt
] coordinates {
    ({72.70 + \dx},0) ({72.70 + \dx},-0.900000)
};


==> plots/violin_ret/eurosat.tex <==
% ======================================================
% Baseline (x-axis at y=0)
% ======================================================
\addplot[
    name path=baseline,
    draw=none
]
coordinates {(21.83,0) (72.65,0)};

% ======================================================
% DEFAULT
% ======================================================

% ---- DS-Temp (top half) ----
\addplot[
    name path=ds_default_top,
    smooth,
    draw=\dstempcol,
    dashed,
    line width=0.8pt
] coordinates {
    ({21.83 - \dx}, 0.000000)
    ({26.91 - \dx}, 0.028937)
    ({37.08 - \dx}, 0.173623)
    ({47.24 - \dx}, 0.173623)
    ({57.40 - \dx}, 0.028937)
    ({67.57 - \dx}, 0.086812)
    ({72.65 - \dx}, 0.000000)
};

\addplot[
    fill=\dstempcol,
    fill opacity=0.2,
]
fill between[
    of=ds_default_top and baseline
];
\addplot[
    draw=\dstempcol,
    dashed,
    dash pattern=on 2pt off 1.4pt,
    dash phase=0pt,
    line width=0.5pt
] coordinates {
    ({45.81 - \dx},0) ({45.81 - \dx},0.900000)
};

% ---- LLaMA (bottom half) ----
\addplot[
    name path=llama_default_bot,
    smooth,
    draw=\llamacol,
    dashed,
    line width=0.8pt
] coordinates {
    ({21.83 - \dx}, -0.000000)
    ({26.91 - \dx}, -0.028937)
    ({37.08 - \dx}, -0.231498)
    ({47.24 - \dx}, -0.144686)
    ({57.40 - \dx}, -0.086812)
    ({67.57 - \dx}, -0.000000)
    ({72.65 - \dx}, -0.000000)
};

\addplot[
    fill=\llamacol,
    fill opacity=0.2,
]
fill between[
    of=llama_default_bot and baseline
];

\addplot[
    draw=\llamacol,
    dashed,
    dash pattern=on 2pt off 1.4pt,
    dash phase=0pt,
    line width=0.5pt
] coordinates {
    (43.24,0) (43.24,-0.900000)
};

% ======================================================
% CENTERED
% ======================================================

% ---- DS-Temp (top half) ----
\addplot[
    name path=ds_white_top,
    smooth,
    draw=\dstempcol,
    solid,
    line width=1.2pt
] coordinates {
    ({21.83 + \dx}, 0.000000)
    ({26.91 + \dx}, 0.028937)
    ({37.08 + \dx}, 0.000000)
    ({47.24 + \dx}, 0.115749)
    ({57.40 + \dx}, 0.202560)
    ({67.57 + \dx}, 0.144686)
    ({72.65 + \dx}, 0.000000)
};

\addplot[
    fill=\dstempcol,
    fill opacity=0.4,
]
fill between[
    of=ds_white_top and baseline
];
\addplot[
    draw=\dstempcol,
    solid,
    line width=0.5pt
] coordinates {
    ({55.26 + \dx},0) ({55.26 + \dx},0.900000)
};

% ---- LLaMA (bottom half) ----
\addplot[
    name path=llama_white_bot,
    smooth,
    draw=\llamacol,
    solid,
    line width=1.2pt
] coordinates {
    ({21.83 + \dx}, -0.000000)
    ({26.91 + \dx}, -0.028937)
    ({37.08 + \dx}, -0.000000)
    ({47.24 + \dx}, -0.115749)
    ({57.40 + \dx}, -0.202560)
    ({67.57 + \dx}, -0.144686)
    ({72.65 + \dx}, -0.000000)
};

\addplot[
    fill=\llamacol,
    fill opacity=0.4,
]
fill between[
    of=llama_white_bot and baseline
];
\addplot[
    draw=\llamacol,
    solid,
    line width=0.5pt
] coordinates {
    ({56.40 + \dx},0) ({56.40 + \dx},-0.900000)
};


==> plots/violin_ret/mlrsnet.tex <==
% ======================================================
% Baseline (x-axis at y=0)
% ======================================================
\addplot[
    name path=baseline,
    draw=none
]
coordinates {(32.97,0) (67.55,0)};

% ======================================================
% DEFAULT
% ======================================================

% ---- DS-Temp (top half) ----
\addplot[
    name path=ds_default_top,
    smooth,
    draw=\dstempcol,
    dashed,
    line width=0.8pt
] coordinates {
    ({32.97 - \dx}, 0.000000)
    ({36.43 - \dx}, 0.000000)
    ({43.34 - \dx}, 0.085054)
    ({50.26 - \dx}, 0.212636)
    ({57.18 - \dx}, 0.212636)
    ({64.09 - \dx}, 0.212636)
    ({67.55 - \dx}, 0.000000)
};

\addplot[
    fill=\dstempcol,
    fill opacity=0.2,
]
fill between[
    of=ds_default_top and baseline
];
\addplot[
    draw=\dstempcol,
    dashed,
    dash pattern=on 2pt off 1.4pt,
    dash phase=0pt,
    line width=0.5pt
] coordinates {
    ({55.59 - \dx},0) ({55.59 - \dx},0.900000)
};

% ---- LLaMA (bottom half) ----
\addplot[
    name path=llama_default_bot,
    smooth,
    draw=\llamacol,
    dashed,
    line width=0.8pt
] coordinates {
    ({32.97 - \dx}, -0.000000)
    ({36.43 - \dx}, -0.085054)
    ({43.34 - \dx}, -0.042527)
    ({50.26 - \dx}, -0.340217)
    ({57.18 - \dx}, -0.212636)
    ({64.09 - \dx}, -0.042527)
    ({67.55 - \dx}, -0.000000)
};

\addplot[
    fill=\llamacol,
    fill opacity=0.2,
]
fill between[
    of=llama_default_bot and baseline
];
\addplot[
    draw=\llamacol,
    dashed,
    dash pattern=on 2pt off 1.4pt,
    dash phase=0pt,
    line width=0.5pt
] coordinates {
    ({50.91 - \dx},0) ({50.91 - \dx},-0.900000)
};

% ======================================================
% CENTERED
% ======================================================

% ---- DS-Temp (top half) ----
\addplot[
    name path=ds_white_top,
    smooth,
    draw=\dstempcol,
    solid,
    line width=1.2pt
] coordinates {
    ({32.97 + \dx}, 0.000000)
    ({36.43 + \dx}, 0.000000)
    ({43.34 + \dx}, 0.000000)
    ({50.26 + \dx}, 0.042527)
    ({57.18 + \dx}, 0.255163)
    ({64.09 + \dx}, 0.425271)
    ({67.55 + \dx}, 0.000000)
};

\addplot[
    fill=\dstempcol,
    fill opacity=0.4,
]
fill between[
    of=ds_white_top and baseline
];
\addplot[
    draw=\dstempcol,
    solid,
    line width=0.5pt
] coordinates {
    ({60.84 + \dx},0) ({60.84 + \dx},0.900000)
};

% ---- LLaMA (bottom half) ----
\addplot[
    name path=llama_white_bot,
    smooth,
    draw=\llamacol,
    solid,
    line width=1.2pt
] coordinates {
    ({32.97 + \dx}, -0.000000)
    ({36.43 + \dx}, -0.000000)
    ({43.34 + \dx}, -0.000000)
    ({50.26 + \dx}, -0.042527)
    ({57.18 + \dx}, -0.340217)
    ({64.09 + \dx}, -0.340217)
    ({67.55 + \dx}, -0.000000)
};

\addplot[
    fill=\llamacol,
    fill opacity=0.4,
]
fill between[
    of=llama_white_bot and baseline
];
\addplot[
    draw=\llamacol,
    solid,
    line width=0.5pt
] coordinates {
    ({60.48 + \dx},0) ({60.48 + \dx},-0.900000)
};


==> plots/violin_ret/optimal31.tex <==
% ======================================================
% Baseline (x-axis at y=0)
% ======================================================
\addplot[
    name path=baseline,
    draw=none
]
coordinates {(50.67,0) (86.98,0)};

% ======================================================
% DEFAULT
% ======================================================

% ---- DS-Temp (top half) ----
\addplot[
    name path=ds_default_top,
    smooth,
    draw=\dstempcol,
    dashed,
    line width=0.8pt
] coordinates {
    ({50.67 - \dx}, 0.000000)
    ({54.30 - \dx}, 0.000000)
    ({61.56 - \dx}, 0.000000)
    ({68.83 - \dx}, 0.162004)
    ({76.09 - \dx}, 0.364508)
    ({83.35 - \dx}, 0.162004)
    ({86.98 - \dx}, 0.000000)
};

\addplot[
    fill=\dstempcol,
    fill opacity=0.2,
]
fill between[
    of=ds_default_top and baseline
];
\addplot[
    draw=\dstempcol,
    dashed,
    dash pattern=on 2pt off 1.4pt,
    dash phase=0pt,
    line width=0.5pt
] coordinates {
    ({75.78 - \dx},0) ({75.78 - \dx},0.900000)
};

% ---- LLaMA (bottom half) ----
\addplot[
    name path=llama_default_bot,
    smooth,
    draw=\llamacol,
    dashed,
    line width=0.8pt
] coordinates {
    ({50.67 - \dx}, -0.000000)
    ({54.30 - \dx}, -0.040501)
    ({61.56 - \dx}, -0.081002)
    ({68.83 - \dx}, -0.364508)
    ({76.09 - \dx}, -0.202505)
    ({83.35 - \dx}, -0.000000)
    ({86.98 - \dx}, -0.000000)
};

\addplot[
    fill=\llamacol,
    fill opacity=0.2,
]
fill between[
    of=llama_default_bot and baseline
];
\addplot[
    draw=\llamacol,
    dashed,
    dash pattern=on 2pt off 1.4pt,
    dash phase=0pt,
    line width=0.5pt
] coordinates {
    ({68.60 - \dx},0) ({68.60 - \dx},-0.900000)
};

% ======================================================
% CENTERED
% ======================================================

% ---- DS-Temp (top half) ----
\addplot[
    name path=ds_white_top,
    smooth,
    draw=\dstempcol,
    solid,
    line width=1.2pt
] coordinates {
    ({50.67 + \dx}, 0.000000)
    ({54.30 + \dx}, 0.000000)
    ({61.56 + \dx}, 0.000000)
    ({68.83 + \dx}, 0.000000)
    ({76.09 + \dx}, 0.324007)
    ({83.35 + \dx}, 0.364508)
    ({86.98 + \dx}, 0.000000)
};

\addplot[
    fill=\dstempcol,
    fill opacity=0.4,
]
fill between[
    of=ds_white_top and baseline
];
\addplot[
    draw=\dstempcol,
    solid,
    line width=0.5pt
] coordinates {
    ({79.84 + \dx},0) ({79.84 + \dx},0.900000)
};

% ---- LLaMA (bottom half) ----
\addplot[
    name path=llama_white_bot,
    smooth,
    draw=\llamacol,
    solid,
    line width=1.2pt
] coordinates {
    ({50.67 + \dx}, -0.000000)
    ({54.30 + \dx}, -0.000000)
    ({61.56 + \dx}, -0.000000)
    ({68.83 + \dx}, -0.000000)
    ({76.09 + \dx}, -0.445510)
    ({83.35 + \dx}, -0.243005)
    ({86.98 + \dx}, -0.000000)
};

\addplot[
    fill=\llamacol,
    fill opacity=0.4,
]
fill between[
    of=llama_white_bot and baseline
];
\addplot[
    draw=\llamacol,
    solid,
    line width=0.5pt
] coordinates {
    ({78.89 + \dx},0) ({78.89 + \dx},-0.900000)
};


==> plots/violin_ret/patternnet.tex <==
% ======================================================
% Baseline (x-axis at y=0)
% ======================================================
\addplot[
    name path=baseline,
    draw=none
]
coordinates {(37.25,0) (81.10,0)};

% ======================================================
% DEFAULT
% ======================================================

% ---- DS-Temp (top half) ----
\addplot[
    name path=ds_default_top,
    smooth,
    draw=\dstempcol,
    dashed,
    line width=0.8pt
] coordinates {
    ({37.25 - \dx}, 0.000000)
    ({41.63 - \dx}, 0.000000)
    ({50.41 - \dx}, 0.067074)
    ({59.17 - \dx}, 0.100610)
    ({67.94 - \dx}, 0.201221)
    ({76.72 - \dx}, 0.201221)
    ({81.10 - \dx}, 0.000000)
};

\addplot[
    fill=\dstempcol,
    fill opacity=0.2,
]
fill between[
    of=ds_default_top and baseline
];
\addplot[
    draw=\dstempcol,
    dashed,
    dash pattern=on 2pt off 1.4pt,
    dash phase=0pt,
    line width=0.5pt
] coordinates {
    ({68.31 - \dx},0) ({68.31 - \dx},0.900000)
};

% ---- LLaMA (bottom half) ----
\addplot[
    name path=llama_default_bot,
    smooth,
    draw=\llamacol,
    dashed,
    line width=0.8pt
] coordinates {
    ({37.25 - \dx}, -0.000000)
    ({41.63 - \dx}, -0.033537)
    ({50.41 - \dx}, -0.033537)
    ({59.17 - \dx}, -0.167684)
    ({67.94 - \dx}, -0.201221)
    ({76.72 - \dx}, -0.134147)
    ({81.10 - \dx}, -0.000000)
};

\addplot[
    fill=\llamacol,
    fill opacity=0.2,
]
fill between[
    of=llama_default_bot and baseline
];
\addplot[
    draw=\llamacol,
    dashed,
    dash pattern=on 2pt off 1.4pt,
    dash phase=0pt,
    line width=0.5pt
] coordinates {
    ({64.77 - \dx},0) ({64.77 - \dx},-0.900000)
};

% ======================================================
% CENTERED
% ======================================================

% ---- DS-Temp (top half) ----
\addplot[
    name path=ds_white_top,
    smooth,
    draw=\dstempcol,
    solid,
    line width=1.2pt
] coordinates {
    ({37.25 + \dx}, 0.000000)
    ({41.63 + \dx}, 0.000000)
    ({50.41 + \dx}, 0.033537)
    ({59.17 + \dx}, 0.033537)
    ({67.94 + \dx}, 0.234758)
    ({76.72 + \dx}, 0.268294)
    ({81.10 + \dx}, 0.000000)
};

\addplot[
    fill=\dstempcol,
    fill opacity=0.4,
]
fill between[
    of=ds_white_top and baseline
];
\addplot[
    draw=\dstempcol,
    solid,
    line width=0.5pt
] coordinates {
    ({71.26 + \dx},0) ({71.26 + \dx},0.900000)
};

% ---- LLaMA (bottom half) ----
\addplot[
    name path=llama_white_bot,
    smooth,
    draw=\llamacol,
    solid,
    line width=1.2pt
] coordinates {
    ({37.25 + \dx}, -0.000000)
    ({41.63 + \dx}, -0.000000)
    ({50.41 + \dx}, -0.033537)
    ({59.17 + \dx}, -0.000000)
    ({67.94 + \dx}, -0.234758)
    ({76.72 + \dx}, -0.301831)
    ({81.10 + \dx}, -0.000000)
};

\addplot[
    fill=\llamacol,
    fill opacity=0.4,
]
fill between[
    of=llama_white_bot and baseline
];
\addplot[
    draw=\llamacol,
    solid,
    line width=0.5pt
] coordinates {
    ({71.72 + \dx},0) ({71.72 + \dx},-0.900000)
};


==> plots/violin_ret/resisc45.tex <==
% ======================================================
% Baseline (x-axis at y=0)
% ======================================================
\addplot[
    name path=baseline,
    draw=none
]
coordinates {(39.22,0) (78.14,0)};

% ======================================================
% DEFAULT
% ======================================================

% ---- DS-Temp (top half) ----
\addplot[
    name path=ds_default_top,
    smooth,
    draw=\dstempcol,
    dashed,
    line width=0.8pt
] coordinates {
    ({39.22 - \dx}, 0.000000)
    ({43.11 - \dx}, 0.000000)
    ({50.90 - \dx}, 0.037785)
    ({58.68 - \dx}, 0.188924)
    ({66.46 - \dx}, 0.226709)
    ({74.25 - \dx}, 0.188924)
    ({78.14 - \dx}, 0.000000)
};

\addplot[
    fill=\dstempcol,
    fill opacity=0.2,
]
fill between[
    of=ds_default_top and baseline
];
\addplot[
    draw=\dstempcol,
    dashed,
    dash pattern=on 2pt off 1.4pt,
    dash phase=0pt,
    line width=0.5pt
] coordinates {
    ({65.13 - \dx},0) ({65.13 - \dx},0.900000)
};

% ---- LLaMA (bottom half) ----
\addplot[
    name path=llama_default_bot,
    smooth,
    draw=\llamacol,
    dashed,
    line width=0.8pt
] coordinates {
    ({39.22 - \dx}, -0.000000)
    ({43.11 - \dx}, -0.037785)
    ({50.90 - \dx}, -0.075570)
    ({58.68 - \dx}, -0.264494)
    ({66.46 - \dx}, -0.264494)
    ({74.25 - \dx}, -0.000000)
    ({78.14 - \dx}, -0.000000)
};

\addplot[
    fill=\llamacol,
    fill opacity=0.2,
]
fill between[
    of=llama_default_bot and baseline
];
\addplot[
    draw=\llamacol,
    dashed,
    dash pattern=on 2pt off 1.4pt,
    dash phase=0pt,
    line width=0.5pt
] coordinates {
    ({59.31 - \dx},0) ({59.31 - \dx},-0.900000)
};

% ======================================================
% CENTERED
% ======================================================

% ---- DS-Temp (top half) ----
\addplot[
    name path=ds_white_top,
    smooth,
    draw=\dstempcol,
    solid,
    line width=1.2pt
] coordinates {
    ({39.22 + \dx}, 0.000000)
    ({43.11 + \dx}, 0.000000)
    ({50.90 + \dx}, 0.000000)
    ({58.68 + \dx}, 0.037785)
    ({66.46 + \dx}, 0.302279)
    ({74.25 + \dx}, 0.302279)
    ({78.14 + \dx}, 0.000000)
};

\addplot[
    fill=\dstempcol,
    fill opacity=0.4,
]
fill between[
    of=ds_white_top and baseline
];
\addplot[
    draw=\dstempcol,
    solid,
    line width=0.5pt
] coordinates {
    ({69.42 + \dx},0) ({69.42 + \dx},0.900000)
};

% ---- LLaMA (bottom half) ----
\addplot[
    name path=llama_white_bot,
    smooth,
    draw=\llamacol,
    solid,
    line width=1.2pt
] coordinates {
    ({39.22 + \dx}, -0.000000)
    ({43.11 + \dx}, -0.000000)
    ({50.90 + \dx}, -0.000000)
    ({58.68 + \dx}, -0.037785)
    ({66.46 + \dx}, -0.264494)
    ({74.25 + \dx}, -0.340064)
    ({78.14 + \dx}, -0.000000)
};

\addplot[
    fill=\llamacol,
    fill opacity=0.4,
]
fill between[
    of=llama_white_bot and baseline
];
\addplot[
    draw=\llamacol,
    solid,
    line width=0.5pt
] coordinates {
    ({70.08 + \dx},0) ({70.08 + \dx},-0.900000)
};


==> plots/violin_ret/rsc11.tex <==
% ======================================================
% Baseline (x-axis at y=0)
% ======================================================
\addplot[
    name path=baseline,
    draw=none
]
coordinates {(45.10,0) (78.59,0)};

% ======================================================
% DEFAULT
% ======================================================

% ---- DS-Temp (top half) ----
\addplot[
    name path=ds_default_top,
    smooth,
    draw=\dstempcol,
    dashed,
    line width=0.8pt
] coordinates {
    ({45.10 - \dx}, 0.000000)
    ({48.45 - \dx}, 0.043911)
    ({55.15 - \dx}, 0.043911)
    ({61.84 - \dx}, 0.043911)
    ({68.54 - \dx}, 0.351290)
    ({75.24 - \dx}, 0.263468)
    ({78.59 - \dx}, 0.000000)
};

\addplot[
    fill=\dstempcol,
    fill opacity=0.2,
]
fill between[
    of=ds_default_top and baseline
];
\addplot[
    draw=\dstempcol,
    dashed,
    dash pattern=on 2pt off 1.4pt,
    dash phase=0pt,
    line width=0.5pt
] coordinates {
    ({67.78 - \dx},0) ({67.78 - \dx},0.900000)
};

% ---- LLaMA (bottom half) ----
\addplot[
    name path=llama_default_bot,
    smooth,
    draw=\llamacol,
    dashed,
    line width=0.8pt
] coordinates {
    ({45.10 - \dx}, -0.000000)
    ({48.45 - \dx}, -0.087823)
    ({55.15 - \dx}, -0.043911)
    ({61.84 - \dx}, -0.175645)
    ({68.54 - \dx}, -0.439113)
    ({75.24 - \dx}, -0.000000)
    ({78.59 - \dx}, -0.000000)
};

\addplot[
    fill=\llamacol,
    fill opacity=0.2,
]
fill between[
    of=llama_default_bot and baseline
];
\addplot[
    draw=\llamacol,
    dashed,
    dash pattern=on 2pt off 1.4pt,
    dash phase=0pt,
    line width=0.5pt
] coordinates {
    ({64.04 - \dx},0) ({64.04 - \dx},-0.900000)
};

% ======================================================
% CENTERED
% ======================================================

% ---- DS-Temp (top half) ----
\addplot[
    name path=ds_white_top,
    smooth,
    draw=\dstempcol,
    solid,
    line width=1.2pt
] coordinates {
    ({45.10 + \dx}, 0.000000)
    ({48.45 + \dx}, 0.000000)
    ({55.15 + \dx}, 0.000000)
    ({61.84 + \dx}, 0.000000)
    ({68.54 + \dx}, 0.175645)
    ({75.24 + \dx}, 0.570846)
    ({78.59 + \dx}, 0.000000)
};

\addplot[
    fill=\dstempcol,
    fill opacity=0.4,
]
fill between[
    of=ds_white_top and baseline
];
\addplot[
    draw=\dstempcol,
    solid,
    line width=0.5pt
] coordinates {
    ({74.21 + \dx},0) ({74.21 + \dx},0.900000)
};

% ---- LLaMA (bottom half) ----
\addplot[
    name path=llama_white_bot,
    smooth,
    draw=\llamacol,
    solid,
    line width=1.2pt
] coordinates {
    ({45.10 + \dx}, -0.000000)
    ({48.45 + \dx}, -0.000000)
    ({55.15 + \dx}, -0.000000)
    ({61.84 + \dx}, -0.000000)
    ({68.54 + \dx}, -0.131734)
    ({75.24 + \dx}, -0.614758)
    ({78.59 + \dx}, -0.000000)
};

\addplot[
    fill=\llamacol,
    fill opacity=0.4,
]
fill between[
    of=llama_white_bot and baseline
];
\addplot[
    draw=\llamacol,
    solid,
    line width=0.5pt
] coordinates {
    ({73.98 + \dx},0) ({73.98 + \dx},-0.900000)
};


==> plots/violin_ret/rsicb128.tex <==
% ======================================================
% Baseline (x-axis at y=0)
% ======================================================
\addplot[
    name path=baseline,
    draw=none
]
coordinates {(14.69,0) (50.42,0)};

% ======================================================
% DEFAULT
% ======================================================

% ---- DS-Temp (top half) ----
\addplot[
    name path=ds_default_top,
    smooth,
    draw=\dstempcol,
    dashed,
    line width=0.8pt
] coordinates {
    ({14.69 - \dx}, 0.000000)
    ({18.26 - \dx}, 0.123475)
    ({25.41 - \dx}, 0.246950)
    ({32.55 - \dx}, 0.164633)
    ({39.70 - \dx}, 0.123475)
    ({46.85 - \dx}, 0.041158)
    ({50.42 - \dx}, 0.000000)
};

\addplot[
    fill=\dstempcol,
    fill opacity=0.2,
]
fill between[
    of=ds_default_top and baseline
];
\addplot[
    draw=\dstempcol,
    dashed,
    dash pattern=on 2pt off 1.4pt,
    dash phase=0pt,
    line width=0.5pt
] coordinates {
    ({29.46 - \dx},0) ({29.46 - \dx},0.900000)
};

% ---- LLaMA (bottom half) ----
\addplot[
    name path=llama_default_bot,
    smooth,
    draw=\llamacol,
    dashed,
    line width=0.8pt
] coordinates {
    ({14.69 - \dx}, -0.000000)
    ({18.26 - \dx}, -0.246950)
    ({25.41 - \dx}, -0.288109)
    ({32.55 - \dx}, -0.123475)
    ({39.70 - \dx}, -0.041158)
    ({46.85 - \dx}, -0.000000)
    ({50.42 - \dx}, -0.000000)
};

\addplot[
    fill=\llamacol,
    fill opacity=0.2,
]
fill between[
    of=llama_default_bot and baseline
];
\addplot[
    draw=\llamacol,
    dashed,
    dash pattern=on 2pt off 1.4pt,
    dash phase=0pt,
    line width=0.5pt
] coordinates {
    ({24.78 - \dx},0) ({24.78 - \dx},-0.900000)
};

% ======================================================
% CENTERED
% ======================================================

% ---- DS-Temp (top half) ----
\addplot[
    name path=ds_white_top,
    smooth,
    draw=\dstempcol,
    solid,
    line width=1.2pt
] coordinates {
    ({14.69 + \dx}, 0.000000)
    ({18.26 + \dx}, 0.041158)
    ({25.41 + \dx}, 0.000000)
    ({32.55 + \dx}, 0.205792)
    ({39.70 + \dx}, 0.288109)
    ({46.85 + \dx}, 0.164633)
    ({50.42 + \dx}, 0.000000)
};

\addplot[
    fill=\dstempcol,
    fill opacity=0.4,
]
fill between[
    of=ds_white_top and baseline
];
\addplot[
    draw=\dstempcol,
    solid,
    line width=0.5pt
] coordinates {
    ({37.81 + \dx},0) ({37.81 + \dx},0.900000)
};

% ---- LLaMA (bottom half) ----
\addplot[
    name path=llama_white_bot,
    smooth,
    draw=\llamacol,
    solid,
    line width=1.2pt
] coordinates {
    ({14.69 + \dx}, -0.000000)
    ({18.26 + \dx}, -0.000000)
    ({25.41 + \dx}, -0.041158)
    ({32.55 + \dx}, -0.164633)
    ({39.70 + \dx}, -0.329267)
    ({46.85 + \dx}, -0.164633)
    ({50.42 + \dx}, -0.000000)
};

\addplot[
    fill=\llamacol,
    fill opacity=0.4,
]
fill between[
    of=llama_white_bot and baseline
];
\addplot[
    draw=\llamacol,
    solid,
    line width=0.5pt
] coordinates {
    ({38.20 + \dx},0) ({38.20 + \dx},-0.900000)
};


==> plots/violin_ret/rsicb256.tex <==
% ======================================================
% Baseline (x-axis at y=0)
% ======================================================
\addplot[
    name path=baseline,
    draw=none
]
coordinates {(28.20,0) (59.02,0)};

% ======================================================
% DEFAULT
% ======================================================

% ---- DS-Temp (top half) ----
\addplot[
    name path=ds_default_top,
    smooth,
    draw=\dstempcol,
    dashed,
    line width=0.8pt
] coordinates {
    ({28.20 - \dx}, 0.000000)
    ({31.28 - \dx}, 0.047715)
    ({37.45 - \dx}, 0.238577)
    ({43.61 - \dx}, 0.238577)
    ({49.77 - \dx}, 0.143146)
    ({55.94 - \dx}, 0.143146)
    ({59.02 - \dx}, 0.000000)
};

\addplot[
    fill=\dstempcol,
    fill opacity=0.2,
]
fill between[
    of=ds_default_top and baseline
];
\addplot[
    draw=\dstempcol,
    dashed,
    dash pattern=on 2pt off 1.4pt,
    dash phase=0pt,
    line width=0.5pt
] coordinates {
    ({43.94 - \dx},0) ({43.94 - \dx},0.900000)
};

% ---- LLaMA (bottom half) ----
\addplot[
    name path=llama_default_bot,
    smooth,
    draw=\llamacol,
    dashed,
    line width=0.8pt
] coordinates {
    ({28.20 - \dx}, -0.000000)
    ({31.28 - \dx}, -0.238577)
    ({37.45 - \dx}, -0.334008)
    ({43.61 - \dx}, -0.190862)
    ({49.77 - \dx}, -0.047715)
    ({55.94 - \dx}, -0.000000)
    ({59.02 - \dx}, -0.000000)
};

\addplot[
    fill=\llamacol,
    fill opacity=0.2,
]
fill between[
    of=llama_default_bot and baseline
];
\addplot[
    draw=\llamacol,
    dashed,
    dash pattern=on 2pt off 1.4pt,
    dash phase=0pt,
    line width=0.5pt
] coordinates {
    ({37.41 - \dx},0) ({37.41 - \dx},-0.900000)
};

% ======================================================
% CENTERED
% ======================================================

% ---- DS-Temp (top half) ----
\addplot[
    name path=ds_white_top,
    smooth,
    draw=\dstempcol,
    solid,
    line width=1.2pt
] coordinates {
    ({28.20 + \dx}, 0.000000)
    ({31.28 + \dx}, 0.000000)
    ({37.45 + \dx}, 0.000000)
    ({43.61 + \dx}, 0.095431)
    ({49.77 + \dx}, 0.286292)
    ({55.94 + \dx}, 0.429438)
    ({59.02 + \dx}, 0.000000)
};

\addplot[
    fill=\dstempcol,
    fill opacity=0.4,
]
fill between[
    of=ds_white_top and baseline
];
\addplot[
    draw=\dstempcol,
    solid,
    line width=0.5pt
] coordinates {
    ({52.66 + \dx},0) ({52.66 + \dx},0.900000)
};

% ---- LLaMA (bottom half) ----
\addplot[
    name path=llama_white_bot,
    smooth,
    draw=\llamacol,
    solid,
    line width=1.2pt
] coordinates {
    ({28.20 + \dx}, -0.000000)
    ({31.28 + \dx}, -0.000000)
    ({37.45 + \dx}, -0.047715)
    ({43.61 + \dx}, -0.000000)
    ({49.77 + \dx}, -0.286292)
    ({55.94 + \dx}, -0.477154)
    ({59.02 + \dx}, -0.000000)
};

\addplot[
    fill=\llamacol,
    fill opacity=0.4,
]
fill between[
    of=llama_white_bot and baseline
];
\addplot[
    draw=\llamacol,
    solid,
    line width=0.5pt
] coordinates {
    ({52.37 + \dx},0) ({52.37 + \dx},-0.900000)
};


==> plots/violin_ret/rsscn7.tex <==
% ======================================================
% Baseline (x-axis at y=0)
% ======================================================
\addplot[
    name path=baseline,
    draw=none
]
coordinates {(40.83,0) (85.05,0)};

% ======================================================
% DEFAULT
% ======================================================

% ---- DS-Temp (top half) ----
\addplot[
    name path=ds_default_top,
    smooth,
    draw=\dstempcol,
    dashed,
    line width=0.8pt
] coordinates {
    ({40.83 - \dx}, 0.000000)
    ({45.25 - \dx}, 0.000000)
    ({54.10 - \dx}, 0.099769)
    ({62.94 - \dx}, 0.099769)
    ({71.78 - \dx}, 0.365818)
    ({80.63 - \dx}, 0.000000)
    ({85.05 - \dx}, 0.000000)
};

\addplot[
    fill=\dstempcol,
    fill opacity=0.2,
]
fill between[
    of=ds_default_top and baseline
];
\addplot[
    draw=\dstempcol,
    dashed,
    dash pattern=on 2pt off 1.4pt,
    dash phase=0pt,
    line width=0.5pt
] coordinates {
    ({66.60 - \dx},0) ({66.60 - \dx},0.900000)
};

% ---- LLaMA (bottom half) ----
\addplot[
    name path=llama_default_bot,
    smooth,
    draw=\llamacol,
    dashed,
    line width=0.8pt
] coordinates {
    ({40.83 - \dx}, -0.000000)
    ({45.25 - \dx}, -0.033256)
    ({54.10 - \dx}, -0.066512)
    ({62.94 - \dx}, -0.232793)
    ({71.78 - \dx}, -0.232793)
    ({80.63 - \dx}, -0.000000)
    ({85.05 - \dx}, -0.000000)
};

\addplot[
    fill=\llamacol,
    fill opacity=0.2,
]
fill between[
    of=llama_default_bot and baseline
];
\addplot[
    draw=\llamacol,
    dashed,
    dash pattern=on 2pt off 1.4pt,
    dash phase=0pt,
    line width=0.5pt
] coordinates {
    ({64.42 - \dx},0) ({64.42 - \dx},-0.900000)
};

% ======================================================
% CENTERED
% ======================================================

% ---- DS-Temp (top half) ----
\addplot[
    name path=ds_white_top,
    smooth,
    draw=\dstempcol,
    solid,
    line width=1.2pt
] coordinates {
    ({40.83 + \dx}, 0.000000)
    ({45.25 + \dx}, 0.000000)
    ({54.10 + \dx}, 0.000000)
    ({62.94 + \dx}, 0.099769)
    ({71.78 + \dx}, 0.099769)
    ({80.63 + \dx}, 0.365818)
    ({85.05 + \dx}, 0.000000)
};

\addplot[
    fill=\dstempcol,
    fill opacity=0.4,
]
fill between[
    of=ds_white_top and baseline
];
\addplot[
    draw=\dstempcol,
    solid,
    line width=0.5pt
] coordinates {
    ({74.75 + \dx},0) ({74.75 + \dx},0.900000)
};

% ---- LLaMA (bottom half) ----
\addplot[
    name path=llama_white_bot,
    smooth,
    draw=\llamacol,
    solid,
    line width=1.2pt
] coordinates {
    ({40.83 + \dx}, -0.000000)
    ({45.25 + \dx}, -0.000000)
    ({54.10 + \dx}, -0.000000)
    ({62.94 + \dx}, -0.000000)
    ({71.78 + \dx}, -0.133025)
    ({80.63 + \dx}, -0.432330)
    ({85.05 + \dx}, -0.000000)
};

\addplot[
    fill=\llamacol,
    fill opacity=0.4,
]
fill between[
    of=llama_white_bot and baseline
];
\addplot[
    draw=\llamacol,
    solid,
    line width=0.5pt
] coordinates {
    ({79.49 + \dx},0) ({79.49 + \dx},-0.900000)
};


==> plots/violin_ret/siriwhu.tex <==
% ======================================================
% Baseline (x-axis at y=0)
% ======================================================
\addplot[
    name path=baseline,
    draw=none
]
coordinates {(41.60,0) (72.44,0)};

% ======================================================
% DEFAULT
% ======================================================

% ---- DS-Temp (top half) ----
\addplot[
    name path=ds_default_top,
    smooth,
    draw=\dstempcol,
    dashed,
    line width=0.8pt
] coordinates {
    ({41.60 - \dx}, 0.000000)
    ({44.68 - \dx}, 0.047684)
    ({50.85 - \dx}, 0.190738)
    ({57.02 - \dx}, 0.381476)
    ({63.19 - \dx}, 0.190738)
    ({69.36 - \dx}, 0.000000)
    ({72.44 - \dx}, 0.000000)
};

\addplot[
    fill=\dstempcol,
    fill opacity=0.2,
]
fill between[
    of=ds_default_top and baseline
];
\addplot[
    draw=\dstempcol,
    dashed,
    dash pattern=on 2pt off 1.4pt,
    dash phase=0pt,
    line width=0.5pt
] coordinates {
    ({56.49 - \dx},0) ({56.49 - \dx},0.900000)
};

% ---- LLaMA (bottom half) ----
\addplot[
    name path=llama_default_bot,
    smooth,
    draw=\llamacol,
    dashed,
    line width=0.8pt
] coordinates {
    ({41.60 - \dx}, -0.000000)
    ({44.68 - \dx}, -0.143053)
    ({50.85 - \dx}, -0.333791)
    ({57.02 - \dx}, -0.190738)
    ({63.19 - \dx}, -0.143053)
    ({69.36 - \dx}, -0.000000)
    ({72.44 - \dx}, -0.000000)
};

\addplot[
    fill=\llamacol,
    fill opacity=0.2,
]
fill between[
    of=llama_default_bot and baseline
];
\addplot[
    draw=\llamacol,
    dashed,
    dash pattern=on 2pt off 1.4pt,
    dash phase=0pt,
    line width=0.5pt
] coordinates {
    ({52.91 - \dx},0) ({52.91 - \dx},-0.900000)
};

% ======================================================
% CENTERED
% ======================================================

% ---- DS-Temp (top half) ----
\addplot[
    name path=ds_white_top,
    smooth,
    draw=\dstempcol,
    solid,
    line width=1.2pt
] coordinates {
    ({41.60 + \dx}, 0.000000)
    ({44.68 + \dx}, 0.000000)
    ({50.85 + \dx}, 0.000000)
    ({57.02 + \dx}, 0.000000)
    ({63.19 + \dx}, 0.286107)
    ({69.36 + \dx}, 0.524529)
    ({72.44 + \dx}, 0.000000)
};

\addplot[
    fill=\dstempcol,
    fill opacity=0.4,
]
fill between[
    of=ds_white_top and baseline
];
\addplot[
    draw=\dstempcol,
    solid,
    line width=0.5pt
] coordinates {
    ({67.26 + \dx},0) ({67.26 + \dx},0.900000)
};

% ---- LLaMA (bottom half) ----
\addplot[
    name path=llama_white_bot,
    smooth,
    draw=\llamacol,
    solid,
    line width=1.2pt
] coordinates {
    ({41.60 + \dx}, -0.000000)
    ({44.68 + \dx}, -0.000000)
    ({50.85 + \dx}, -0.000000)
    ({57.02 + \dx}, -0.000000)
    ({63.19 + \dx}, -0.286107)
    ({69.36 + \dx}, -0.524529)
    ({72.44 + \dx}, -0.000000)
};

\addplot[
    fill=\llamacol,
    fill opacity=0.4,
]
fill between[
    of=llama_white_bot and baseline
];
\addplot[
    draw=\llamacol,
    solid,
    line width=0.5pt
] coordinates {
    ({67.43 + \dx},0) ({67.43 + \dx},-0.900000)
};


==> plots/violin_ret/whurs19.tex <==
% ======================================================
% Baseline (x-axis at y=0)
% ======================================================
\addplot[
    name path=baseline,
    draw=none
]
coordinates {(46.03,0) (96.61,0)};

% ======================================================
% DEFAULT
% ======================================================

% ---- DS-Temp (top half) ----
\addplot[
    name path=ds_default_top,
    smooth,
    draw=\dstempcol,
    dashed,
    line width=0.8pt
] coordinates {
    ({46.03 - \dx}, 0.000000)
    ({51.09 - \dx}, 0.029075)
    ({61.20 - \dx}, 0.000000)
    ({71.32 - \dx}, 0.000000)
    ({81.44 - \dx}, 0.348894)
    ({91.55 - \dx}, 0.116298)
    ({96.61 - \dx}, 0.000000)
};

\addplot[
    fill=\dstempcol,
    fill opacity=0.2,
]
fill between[
    of=ds_default_top and baseline
];
\addplot[
    draw=\dstempcol,
    dashed,
    dash pattern=on 2pt off 1.4pt,
    dash phase=0pt,
    line width=0.5pt
] coordinates {
    ({81.54 - \dx},0) ({81.54 - \dx},0.900000)
};

% ---- LLaMA (bottom half) ----
\addplot[
    name path=llama_default_bot,
    smooth,
    draw=\llamacol,
    dashed,
    line width=0.8pt
] coordinates {
    ({46.03 - \dx}, -0.000000)
    ({51.09 - \dx}, -0.029075)
    ({61.20 - \dx}, -0.000000)
    ({71.32 - \dx}, -0.290745)
    ({81.44 - \dx}, -0.174447)
    ({91.55 - \dx}, -0.000000)
    ({96.61 - \dx}, -0.000000)
};

\addplot[
    fill=\llamacol,
    fill opacity=0.2,
]
fill between[
    of=llama_default_bot and baseline
];
\addplot[
    draw=\llamacol,
    dashed,
    dash pattern=on 2pt off 1.4pt,
    dash phase=0pt,
    line width=0.5pt
] coordinates {
    ({73.94 - \dx},0) ({73.94 - \dx},-0.900000)
};

% ======================================================
% CENTERED
% ======================================================

% ---- DS-Temp (top half) ----
\addplot[
    name path=ds_white_top,
    smooth,
    draw=\dstempcol,
    solid,
    line width=1.2pt
] coordinates {
    ({46.03 + \dx}, 0.000000)
    ({51.09 + \dx}, 0.000000)
    ({61.20 + \dx}, 0.000000)
    ({71.32 + \dx}, 0.000000)
    ({81.44 + \dx}, 0.087224)
    ({91.55 + \dx}, 0.407043)
    ({96.61 + \dx}, 0.000000)
};

\addplot[
    fill=\dstempcol,
    fill opacity=0.4,
]
fill between[
    of=ds_white_top and baseline
];
\addplot[
    draw=\dstempcol,
    solid,
    line width=0.5pt
] coordinates {
    ({89.82 + \dx},0) ({89.82 + \dx},0.900000)
};

% ---- LLaMA (bottom half) ----
\addplot[
    name path=llama_white_bot,
    smooth,
    draw=\llamacol,
    solid,
    line width=1.2pt
] coordinates {
    ({46.03 + \dx}, -0.000000)
    ({51.09 + \dx}, -0.000000)
    ({61.20 + \dx}, -0.000000)
    ({71.32 + \dx}, -0.000000)
    ({81.44 + \dx}, -0.116298)
    ({91.55 + \dx}, -0.377969)
    ({96.61 + \dx}, -0.000000)
};

\addplot[
    fill=\llamacol,
    fill opacity=0.4,
]
fill between[
    of=llama_white_bot and baseline
];
\addplot[
    draw=\llamacol,
    solid,
    line width=0.5pt
] coordinates {
    ({88.48 + \dx},0) ({88.48 + \dx},-0.900000)
};

